On Perceived Emotion in Expressive Piano Performance: Further Experimental Evidence for the Relevance of Mid-level Perceptual Features

Despite recent advances in audio content-based music emotion recognition, a question that remains to be explored is whether an algorithm can reliably discern emotional or expressive qualities between different performances of the same piece. In the present work, we analyze several sets of features on their effectiveness in predicting arousal and valence of six different performances (by six famous pianists) of Bach's Well-Tempered Clavier Book 1. These features include low-level acoustic features, score-based features, features extracted using a pre-trained emotion model, and Mid-level perceptual features. We compare their predictive power by evaluating them on several experiments designed to test performance-wise or piece-wise variations of emotion. We find that Mid-level features show significant contribution in performance-wise variation of both arousal and valence -- even better than the pre-trained emotion model. Our findings add to the evidence of Mid-level perceptual features being an important representation of musical attributes for several tasks -- specifically, in this case, for capturing the expressive aspects of music that manifest as perceived emotion of a musical performance.

==> perf_wise_ml_features_corr.tex <==
\begin{table}[h]
\small
\resizebox{\columnwidth}{!}{%
  \begin{tabular}{l|r|r|r|r}
    \multirow{2}{*}{} &
      \multicolumn{2}{c|}{Arousal} &
      \multicolumn{2}{c}{Valence} \\
    
    Mid-level Feature & Corr & $p<0.1$ & Corr & $p<0.1$  \\
    \hline
    melodiousness & \textbf{0.70} & \textbf{62.5\%} & 0.48 & 20.8\%  \\
    articulation & \textbf{0.75} & \textbf{66.7\%} & 0.51 & 22.9\%  \\
    rhythm complexity & 0.61 & 45.8\% & 0.42 & 12.5\%  \\
    rhythm stability & 0.57 & 33.3\% & 0.53 & 35.4\%  \\
    dissonance & 0.67 & 47.9\% & 0.47 & 22.9\%  \\
    tonal stability & 0.47 & 18.8\% & 0.55 & 29.2\%  \\
    minorness & 0.44 & 18.8\% & \textbf{0.78} & \textbf{66.7\%}  \\

  \end{tabular}%
  }
  \caption{Feature-prediction correlations for performances of each piece, averaged over all pieces. The p<0.1 column shows what percentage of pieces had correlations with significance level better than 0.1. \shreyan{Should I make these tables for other feature sets (emotion features and low-level features)? It will take space, and only LL set has a feature that is > 50\% }}
\end{table}
